How Developers Experience Debugging Unfamiliar Codebases with Code Tours Generated and Evaluated by Local LLMs

Code tours are interactive, onboarding documentation to guide developers through a codebase. Large Language Models (LLMs) can automatically synthesize code tours. Prior work on code tour generation has not studied developer experience or trust calibration when debugging unfamiliar codebases with code tours generated and evaluated by open-weight LLMs. This study surveys how the properties of components in open-weight LLM-authored code tours influence developers' experiences when debugging unfamiliar codebases. We built a pipeline that generated and evaluated code tours from real reproducible bugs. 26 developers with varying backgrounds participated in a user study. In total, 26 code tours were authored from real Java bugs mined from 2025 GitHub commits, with each tour independently judged by two different LLMs, resulting in 52 evaluated configurations. Participants thought aloud as they explored each tour. Three authors qualitatively coded the interviews to identify recurring themes. Developers generally preferred tours that scaled detail with the code length, avoided merely restating code, were easily scannable, and adopted a guiding tone. However, some preferences were mutually exclusive, such as the use of imperative mood. Stack traces were often insufficient to identify all steps developers found relevant. Developers also trusted descriptions they perceived as human-written more than those they believed were AI-generated. Finally, LLM-generated annotations of tour quality were unreliable: sycophancy, confabulation, and incoherence were pervasive. This work lays a basis for future research on fine-tuning open-weight models for code tour generation, personalizing generation to accommodate diverging preferences, selecting relevant steps beyond stack traces, calibrating users' trust to avoid both disuse and misuse, and improving open-weight LLMs' ability to be more trustworthy evaluators

==> tours/11.tex <==
\begin{codetour}{3}{\textbf{Code Tour 11 (Medblocks-openFHIR, commit fdaa..., )} generated by \qwCode. The tour covers how to create a conditional FHIR path (a standard for exchanging healthcare resources). The test fails because of a \texttt{ComparisonFailure} due to incorrectly emitting a substring check (\texttt{.contains('bd')}) instead of (\texttt{= 'bd'}) for conditional \texttt{.where} clauses. The structure of the description is noteworthy because it blends natural language with code excerpts.
}{fig:ct-11}
\setcounter{ctstep}{2}
  % -------- Step 3 --------
  \begin{codestep}{OpenFhirStringUtils.java — constructFhirPathWithConditions()}
    \begin{lstlisting}[style=javastyle]
public String constructFhirPathWithConditions(final String originalFhirPath,
                                              final String parentPath,
                                              final Condition condition,
                                              final String resource) {
    // [...] Skipping 23 lines
    if (actualConditionTargetRoot.startsWith(resource) && withParentsWhereInPlace.equals(originalFhirPath)) {
        // [...] Skipping 8 lines
        final String whereClause =
                ".where(" + remainingToAdd + condition.getTargetAttribute() + ".toString().contains('"
                        + getStringFromCriteria(condition.getCriteria()).getCode() + "')" + (negate ? "=false" : "")
                        + ")";
        final String remainingItemsFromParent = originalFhirPath.replace(commonPath, "");
        return commonPath + whereClause + remainingItemsFromParent;
    } else {
        // then do your own where path
        final String whereClause =
                ".where(" + condition.getTargetAttribute() + ".toString().contains('" + getStringFromCriteria(
                        condition.getCriteria()).getCode() + "')" + (negate ? "=false" : "") + ")";
        // then suffix with whatever is left from the children's path
        return withParentsWhereInPlace + whereClause + (StringUtils.isBlank(remainingItems) ? ""
                : (remainingItems.startsWith(".") ? remainingItems : ("." + remainingItems)));
    }
}
    \end{lstlisting}
    \begin{stepnote}
    \textbf{3. constructFhirPathWithConditions in com/medblocks/openfhir/util/OpenFhirStringUtils.java at line 533}

    The method \pinktt{constructFhirPathWithConditions} amends the FHIR path with conditions by constructing a \pinktt{.where} clause based on the provided conditions. Here, the method constructs the FHIR path and appends \pinktt{.where(targetAttribute.toString().contains(conditionCriteria))} to it.
    
    In this specific case, since the condition's operator is not \pinktt{= empty} or \pinktt{!= empty}, it directly invokes the \pinktt{constructFhirPathNoConditions} if the target attribute is null or if no criteria are specified. Otherwise, it constructs the where clause based on the target attribute and criteria (\pinktt{condition.getTargetAttribute() + ".toString().contains('" + getStringFromCriteria(condition.getCriteria()).getCode() + "')}).

    \textbf{Potential Failure Causes:}
    \begin{itemize}
        \item  Incorrect construction of the \pinktt{.where} clause due to mishandled condition attributes or criteria in \pinktt{constructFhirPathWithConditions}.
        \item Using \pinktt{.contains()} instead of \pinktt{.equals()} can lead to unintended behavior if the FHIR path comparison is supposed to be exact.
    \end{itemize}
   

    \end{stepnote}
  \end{codestep}
\end{codetour}

==> tours/33.tex <==
\begin{codetour}{3}{\textbf{Code Tour 33 (package-url-packageurl-java, commit \href{https://github.com/package-url/packageurl-java/commit/f2e1d7aeaf7f0ed6ea72e1f5b8b8b44357a1f240}{f2e1d7a}, trace 8/10)} generated by \mistDev. \textbf{Project.} Package URL is a standardized format for identifying software packages, components, and libraries across different package management systems. \textbf{Commit.} The related commit fixes the URI encoding and decoding that did not properly handle percent-encoding. \textbf{Test.} The test assesses if a \texttt{ValidationException} is properly thrown when there are incomplete non-ASCII characters. In this case, it fails because it throws a  \texttt{StringIndexOutOfBoundsException} instead.\textbf{Tour.} This tour covers how the URIs are decoded, especially how invalid URIs should be handled. Noteworthy because of duplicate steps.
}{fig:ct-33}
\begin{codestep}{PackageURLTest.java — invalidPercentEncoding()}
    \begin{lstlisting}[style=javastyle]
@Test
void invalidPercentEncoding() throws MalformedPackageURLException {
    // Skip 7 lines
    Throwable t3 = assertThrows(ValidationException.class, () -> purl.uriDecode("aaaa%%0A"));
    // Skip 3 lines
}
\end{lstlisting}
\begin{stepnote}
The test \pinktt{invalidPercentEncoding} in \pinktt{PackageURLTest.java} at line 83 aims to validate that invalid percent-encoded strings in a \pinktt{PackageURL} are correctly handled. It expects a \pinktt{ValidationException} to be thrown when an invalid percent-encoded string is encountered during URI decoding. However, the test is failing due to an unexpected \pinktt{StringIndexOutOfBoundsException} instead.

This step is the entry point of the test, where various scenarios of invalid percent-encoded strings are tested. The key assertion here is that the \pinktt{uriDecode} method should throw a \pinktt{ValidationException} with a specific message for each invalid scenario.

To understand why this test is failing, we need to closely examine the \pinktt{uriDecode} method in \pinktt{PackageURL.java} and identify why it's throwing a \pinktt{StringIndexOutOfBoundsException} instead of a \pinktt{ValidationException}.
    \end{stepnote}
\end{codestep}
\begin{codestep}{PackageURLTest.java — invalidPercentEncoding()}
    \begin{lstlisting}[style=javastyle]
@Test
void invalidPercentEncoding() throws MalformedPackageURLException {
    // Skip 7 lines
    Throwable t3 = assertThrows(ValidationException.class, () -> purl.uriDecode("aaaa%%0A"));
    // Skip 3 lines
}
\end{lstlisting}
\begin{stepnote}
The \pinktt{uriDecode} method in \pinktt{PackageURL.java} at line 603 is responsible for decoding a percent-encoded string. This method iterates through each character of the input string. When it encounters a '\%' character, it attempts to read the next two characters as hexadecimal digits, converts them to an integer, and then appends the corresponding character to the result.

However, the method does not handle cases where the percent-encoded string is incomplete or where the hexadecimal digits are invalid. This lack of validation is likely the root cause of the \pinktt{StringIndexOutOfBoundsException} observed in the test.

To fix this issue, we need to add proper validation within the \pinktt{uriDecode} method to ensure that the percent-encoded string is complete and that the hexadecimal digits are valid. If an invalid percent-encoded string is detected, the method should throw a \pinktt{ValidationException} with a descriptive message, aligning with the expectations set in the test.
\end{stepnote}
\end{codestep}
\begin{codestep}{PackageURL.java — uriDecode()}
\begin{lstlisting}[style=javastyle]
public static String uriDecode(String source) {
    int length = source.length();
    StringBuilder builder = new StringBuilder();
    for (int i = 0; i < length; i++) {
        if (source.charAt(i) == '%') {
            String str = source.substring(i + 1, i + 3);
            char c = (char) Integer.parseInt(str, 16);
            builder.append(c);
            i += 2;
// [...] Skip the end (6 lines)
\end{lstlisting}
\begin{stepnote}
Review the \pinktt{uriDecode} method to identify the specific logic that leads to the \pinktt{StringIndexOutOfBoundsException}. The method currently lacks checks to ensure that there are enough characters following a '\%' to form a valid percent-encoded sequence. This oversight results in the \pinktt{StringIndexOutOfBoundsException} when \pinktt{source.substring(i + 1, i + 3)} is called on an incomplete percent-encoded string.

To address this, modify the method to include checks for the length of the string and the validity of the percent-encoded sequences. If an invalid sequence is detected, throw a \pinktt{ValidationException} with an appropriate message, as specified in the test.

Example Fix: [See \Cref{fig:ct-33-fix}]

This fix ensures that the method throws a \pinktt{ValidationException} with a descriptive message when it encounters an incomplete or invalid percent-encoded string, aligning the method's behavior with the test's expectations.
\end{stepnote}
\end{codestep}
\end{codetour}

\begin{lstlisting}[style=javastyle, caption={An example of a fix proposed directly in a code tour (see \Cref{fig:ct-33})}, label={fig:ct-33-fix}]
public static String uriDecode(String source) {
    int length = source.length();
    StringBuilder builder = new StringBuilder();
    for (int i = 0; i < length; i++) {
        if (source.charAt(i) == '%') {
            if (i + 2 >= length) {
                throw new ValidationException("Incomplete percent encoding at offset " + i + " with value '%'");
            }
            String str = source.substring(i + 1, i + 3);
            try {
                char c = (char) Integer.parseInt(str, 16);
                builder.append(c);
            } catch (NumberFormatException e) {
                throw new ValidationException("Invalid percent encoding char at offset " + i + " with value '%'");
            }
            i += 2;
        } else {
            builder.append(source.charAt(i));
        }
    }
    return builder.toString();
}
\end{lstlisting}



==> tours/34.tex <==
\begin{codetour}{3}{\textbf{Code Tour 34 (thibaultmeyer-cuid-java, commit d923...)} generated by \dskCode. The tour covers the creation of CUID (Collision-resistant Unique Identifier), an alternative to UUIDs. The test generates 500,000 random CUIDs and validates them. However, the raised \texttt{AssertionFailure} indicates that at least one CUID failed validation. The structure of the descriptions is noteworthy because it use bullet points.}{fig:ct-34}

% -------- Step 1 --------
  \begin{codestep}{CUIDv1Test.java — validCreation500000()}
    \begin{lstlisting}[style=javastyle]
@Test
void validCreation500000() {
    // Act & Assert
    for (int i = 0; i < 500000; i += 1) {
        final CUID cuid = CUID.randomCUID1();
        Assertions.assertTrue(CUID.isValid(cuid.toString()));
    }
}
    \end{lstlisting}
    \begin{stepnote}

Start with the failing test \pinktt{validCreation500000}.

This test is trying to verify the creation of 500,000 valid Collision Resistant IDs (CUIDs). It generates a random CUID 500,000 times and checks if it's a valid CUID each time. The assertion failure (\pinktt{expected: <true> but was: <false>}) suggests that at least one of the generated CUIDs did not pass the validation.
    \end{stepnote}
  \end{codestep}
  % -------- Step 2 --------
  \begin{codestep}{CUID.java — randomCUID1()}
    \begin{lstlisting}[style=javastyle]
public static CUID randomCUID1() {
    final String timestamp = Long.toString(System.currentTimeMillis(), NUMBER_BASE);
    final String counter = Common.padWithZero(Integer.toString(CUIDv1.nextCounterValue(), NUMBER_BASE), CUIDv1.BLOCK_SIZE);
    final String random = CUIDv1.getRandomBlock() + CUIDv1.getRandomBlock();
    return new CUID(CUIDv1.START_CHARACTER + timestamp + counter + Common.MACHINE_FINGERPRINT + random);
}
    \end{lstlisting}
    \begin{stepnote}
% \tiny
Generating a CUIDv1: \pinktt{randomCUID1()}.

This method creates a random CUID by:
\begin{enumerate}
    \item Converting the current timestamp to a string (\pinktt{timestamp}).
    \item Obtaining the next counter value, padding it with zeros (\pinktt{counter}).
    \item Concatenating two random blocks to form the random part (\pinktt{random}).
    \item Combining and returning the \pinktt{timestamp}, \pinktt{counter}, machine fingerprint, and \pinktt{random} into a new CUID.
\end{enumerate}

The next step in our walkthrough is to explore one of the key components in CUID generation: the random block.
    \end{stepnote}
  \end{codestep}
   % -------- Step 3 --------
  \begin{codestep}{CUID.java — getRandomBlock()}
    \begin{lstlisting}[style=javastyle]
private static String getRandomBlock() {
    return Common.padWithZero(Integer.toString(Common.nextIntValue() * DISCRETE_VALUE, NUMBER_BASE), BLOCK_SIZE);
}
    \end{lstlisting}
    
    \begin{stepnote}
    % \tiny
Random Block Generation: \pinktt{getRandomBlock()}.

This private method generates a random block of data by:

\begin{enumerate}
    \item Getting the next integer value (from a sequence) and multiplying it by a discrete value (\pinktt{DISCRETE\_VALUE}).
    \item Converting this integer to a string using base-32 encoding (\pinktt{NUMBER\_BASE}).
    \item Padding the string with zeros until it meets a required block size (\pinktt{BLOCK\_SIZE}).
\end{enumerate}

The fault seems to originate from here as the random block might not be providing sufficient variability or might have unexpected values. Review the implementation of \pinktt{Common.nextIntValue()} and make sure it can produce distinct values that lead to varied CUIDs. Also check that \pinktt{DISCRETE\_VALUE} and \pinktt{BLOCK\_SIZE} are defined correctly.

By understanding these methods, you can begin to assess why some generated CUIDs are being flagged as invalid by \pinktt{CUID.isValid()}.
    \end{stepnote}
  \end{codestep}
\end{codetour}

==> tours/4.tex <==
\begin{codetour}{3}{\textbf{Code Tour 4 (classgraph-classgraph, commit \href{https://github.com/classgraph/classgraph/commit/fbe61e01e8fadd8cf98dd7891c80e5000c85d6c0}{fbe61e0
}, trace 1/1)} generated by \dskCode. \textbf{Project.} ClassGraph is a classpath and module scanner for JVM languages (it inspects classes, methods, and annotations available at runtime). \textbf{Commit.} This commit fixes \href{https://github.com/classgraph/classgraph/pull/921}{Issue 920} that highlights that when asked for a class's constructors, ClassGraph sometimes returned constructors inherited from the superclass instead of only the class's own constructors, which was confusing when a class declared a non-public constructor with the same signature as one in its superclass. \textbf{Test.} The test checks the modifiers of the no-args constructor of \texttt{ObjectOutputStream}. It fails with an \texttt{AssertionFailedError} because the constructor is reported as \texttt{public} (modifier \texttt{1}) instead of the expected \texttt{protected} (modifier \texttt{4}), revealing that the superclass constructor was returned instead of the actual one. \textbf{Tour.} The tone of this tour is noteworthy because \qwCode{} describes it as somewhat technical, which two participants do not see as a problem. Step 2 is omitted from this document for conciseness.
}{fig:ct-4}
\begin{codestep}{Issue920Test.java — test()}
\begin{lstlisting}[style=javastyle, breaklines=true]
@Test 
void test() {
    MethodInfoList constructors = new ClassGraph().enableAnnotationInfo().enableSystemJarsAndModules().enableClassInfo().enableMethodInfo().scan().getClassInfo("java.io.ObjectOutputStream").getConstructorInfo();
    for (MethodInfo constructor : constructors) {
        if (constructor.getParameterInfo().length == 0) {
            // The no args constructor of ObjectOutputStream is protected
            assertEquals(Modifier.PROTECTED, constructor.getModifiers());
}}}
\end{lstlisting}
\begin{stepnote}
In the test method \pinktt{test} defined in the \pinktt{Issue920Test} class, we are trying to retrieve information about all constructors of the \pinktt{ObjectOutputStream} class. This includes checking if the no-args constructor is protected.
\end{stepnote}
\end{codestep}
% \begin{codestep}{ClassInfo.java — getConstructorInfo()}
% \begin{lstlisting}[style=javastyle, breaklines=true]
% public MethodInfoList getConstructorInfo() {
%     return getMethodInfo(/* methodName = */ null, /* getNormalMethods = */ false, /* getConstructorMethods = */ true, /* getStaticInitializerMethods = */ false);
% }
% \end{lstlisting}
% \begin{stepnote}
% The method \pinktt{getConstructorInfo()} in the \pinktt{ClassInfo} class is responsible for retrieving information on all visible constructors declared by a class or its superclasses. Here, it's being invoked to get details about the constructors of \pinktt{ObjectOutputStream}, including the no-args constructor.
% \end{stepnote}
% \end{codestep}
\stepcounter{ctstep}
\begin{codestep}{ClassInfo.java — getMethodInfo()}
\begin{lstlisting}[style=javastyle, breaklines=true]
private MethodInfoList getMethodInfo(final String methodName, final boolean getNormalMethods, final boolean getConstructorMethods, final boolean getStaticInitializerMethods) {
    if (!scanResult.scanSpec.enableMethodInfo) {
        throw new IllegalArgumentException("Please call ClassGraph#enableMethodInfo() before #scan()");
    }
    // Implement method/constructor overriding
    final MethodInfoList methodInfoList = new MethodInfoList();
    final Set<Entry<String, String>> nameAndTypeDescriptorSet = new HashSet<>();
    for (final ClassInfo ci : getMethodOverrideOrder()) {
        for (final MethodInfo mi : ci.getDeclaredMethodInfo(methodName, getNormalMethods, getConstructorMethods,
                getStaticInitializerMethods)) {
            // If method/constructor has not been overridden by method of same name and type descriptor 
            if (nameAndTypeDescriptorSet.add(new SimpleEntry<>(mi.getName(), mi.getTypeDescriptorStr()))) {
                // Add method/constructor to output order
                methodInfoList.add(mi);
            }
        }
    }
    return methodInfoList;
}
\end{lstlisting}
\begin{stepnote}
Inside the \pinktt{getConstructorInfo()} method, a call is made to \pinktt{getMethodInfo(...)} with specific parameters set to retrieve only constructors. This is done by setting \pinktt{methodName} to \pinktt{null}, \pinktt{getNormalMethods} to \pinktt{false}, \pinktt{getConstructorMethods} to \pinktt{true}, and \pinktt{getStaticInitializerMethods} to \pinktt{false}. It's important that the method info has been enabled for scanning prior to this call, otherwise an exception will be thrown.
\end{stepnote}
\end{codestep}
\end{codetour}

==> tours/6.tex <==
\begin{codetour}{6}{\textbf{Code Tour 6 (ezylang-EvalEx, commit \href{https://github.com/ezylang/EvalEx/commit/942a}{942ad41})} generated by \qwCode. 
\textbf{Project.} EvalEx is an expression evaluator that parses and evaluates expression strings such as \texttt{1 + 2 / (4 * SQRT(4))}. \textbf{Commit.} This commit fixes an index-out-of-bounds error that occurred when a function was called with no parameters, such as \texttt{DT\_DATE\_NEW()}. \textbf{Test.} The test assesses a function call with no arguments. It fails inside \texttt{validatePreEvaluation()}, which checks whether the last entry of the \texttt{parameterValues} array is a string by accessing index \texttt{parameterLength - 1}. When the function has no parameters, the length is \texttt{0}, and the index becomes \texttt{-1}, causing an \texttt{ArrayIndexOutOfBoundsException}. \textbf{Tour.} The tone of this tour is noteworthy for being pedagogical with ending sentences such as "Click 'Next' to understand how the evaluateFunction method is called." Also, the first two steps are duplicated because of a lambda call inside \texttt{assertThrownBy}. Intermediary steps are omitted for conciseness.
}{fig:ct-6}

\begin{codestep}{DateTimeFunctionsTest.java — testDateTimeNewNoParam()}
\begin{lstlisting}[style=javastyle, breaklines=true]
@Test
void testDateTimeNewNoParam() {
    assertThatThrownBy(() -> new Expression("DT_DATE_NEW()").evaluate())
        .isInstanceOf(EvaluationException.class)
        .hasMessage("Not enough parameters for function");
}
\end{lstlisting}
\begin{stepnote}
Welcome to the code tour for tracing the \pinktt{testDateTimeNewNoParam} test failure! In this tour, we'll walk through the execution path that leads to an unexpected ArrayIndexOutOfBoundsException. Click 'Next' to start.
\end{stepnote}
\end{codestep}
\begin{codestep}{DateTimeFunctionsTest.java — testDateTimeNewNoParam()}
\begin{lstlisting}[style=javastyle, breaklines=true]
@Test
void testDateTimeNewNoParam() {
    assertThatThrownBy(() -> new Expression("DT_DATE_NEW()").evaluate())
        .isInstanceOf(EvaluationException.class)
        .hasMessage("Not enough parameters for function");
}
\end{lstlisting}
\begin{stepnote}
Here, we see the \pinktt{testDateTimeNewNoParam} method in the DateTimeFunctionsTest class. This test is designed to verify that the proper exception (\pinktt{EvaluationException}) is thrown when calling the \pinktt{DT\_DATE\_NEW()} function without any parameters. The test expects the message 'Not enough parameters for function'. Click 'Next' to learn what happens next.
\end{stepnote}
\end{codestep}
\stepcounter{ctstep}
\stepcounter{ctstep}
\stepcounter{ctstep}
\begin{codestep}{DateTimeNewFunction.java — validatePreEvaluation()}
\begin{lstlisting}[style=javastyle, breaklines=true]
public void validatePreEvaluation(Token token, EvaluationValue... parameterValues) throws EvaluationException  {
// [...] Skipping 8-10 lines
if (parameterValues[parameterLength - 1].isStringValue()) {
// [...] Skipping lines 10-13 lines
}}
\end{lstlisting}
\begin{stepnote}
This step brings us to \pinktt{validatePreEvaluation}. This method validates parameters passed to the \pinktt{DT\_DATE\_NEW()} function.  It checks the number and types of the provided parameters.

For our test case, no parameters are passed ArrayIndexOutOfBoundsException at index -1). The issue arises because methods such as \pinktt{parameterValues[parameterLength - 1]} attempt to access elements in an array with a negative or out-of-bounds index.

To fix this error, we need to handle the scenario when no parameters are provided and either throw a more appropriate exception (\pinktt{EvaluationException}) or modify the method to accept default parameter values.

Please let me know if you understand how the error occurs. We should address this in your next session!
\end{stepnote}
\end{codestep}
\end{codetour}

==> tours/7.tex <==
% \begin{codetour}{3}{\textbf{Code Tour 7 (fast-pack-JavaFastPFOR, commit \href{https://github.com/fast-pack/JavaFastPFOR/commit/9640566814326385a73c0f794f4c6d36050200d5}{9640566})} generated by \dskCode. 
% \textbf{Project.} JavaFastPFOR is an integer compression library. \textbf{Commit.} This commit fixes variable-byte encoding of large longs (kezako ??) Previously, the branch encoding longs in 9 bytes was unreachable because the condition `val < (1L << 63)` is always false. Only negative longs should be encoded using 10 bytes.
% \textbf{Test.} 

% \textbf{Tour.} Noteworthy because of duplicate steps.
% }{fig:ct-7}
% \end{codetour}
